GIMMICK -- Globally Inclusive Multimodal Multitask Cultural Knowledge Benchmarking

Large Vision-Language Models (LVLMs) have recently gained attention due to their distinctive performance and broad applicability. While it has been previously shown that their efficacy in usage scenarios involving non-Western contexts falls short, existing studies are limited in scope, covering just a narrow range of cultures, focusing exclusively on a small number of cultural aspects, or evaluating a limited selection of models on a single task only. Towards globally inclusive LVLM research, we introduce GIMMICK, an extensive multimodal benchmark designed to assess a broad spectrum of cultural knowledge across 144 countries representing six global macro-regions. GIMMICK comprises six tasks built upon three new datasets that span 728 unique cultural events or facets on which we evaluated 20 LVLMs and 11 LLMs, including five proprietary and 26 open-weight models of all sizes. We systematically examine (1) regional cultural biases, (2) the influence of model size, (3) input modalities, and (4) external cues. Our analyses reveal strong biases toward Western cultures across models and tasks and highlight strong correlations between model size and performance, as well as the effectiveness of multimodal input and external geographic cues. We further find that models have more knowledge of tangible than intangible aspects (e.g., food vs. rituals) and that they excel in recognizing broad cultural origins but struggle with a more nuanced understanding.

==> tables/ckqa_desc_acc_scores.tex <==
\begin{tabular}{llrllrllrllrllrllrllrlr}
\toprule
region & \multicolumn{3}{r}{West EU \& North America} & \multicolumn{3}{r}{East EU} & \multicolumn{3}{r}{Asia \& Pacific} & \multicolumn{3}{r}{Latin-America \& Caribbean} & \multicolumn{3}{r}{Arab} & \multicolumn{3}{r}{Subsaharian Africa} & \multicolumn{4}{r}{Average} \\
combination & I & T & I+T & I & T & I+T & I & T & I+T & I & T & I+T & I & T & I+T & I & T & I+T & I & T & I+T & Avg \\
model &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
\midrule
\rowcolor{gray!20}
GPT-4o & 46.98 & 56.78 & 57.21 & 38.20 & 54.30 & 54.87 & 44.71 & 59.20 & 58.56 & 34.08 & 51.53 & 52.45 & 44.41 & 57.76 & 56.91 & 29.04 & 50.68 & 51.37 & 39.57 & 55.04 & 55.23 & 49.95 \\
Claude 3.5 Sonnet & 43.05 & 56.64 & 55.60 & 35.20 & 55.97 & 50.07 & 39.54 & 59.67 & 54.05 & 26.84 & 53.32 & 49.23 & 41.45 & 56.78 & 53.68 & 24.73 & 50.34 & 44.79 & 35.14 & 55.45 & 51.24 & 47.28 \\
\rowcolor{gray!20}
Gemini Pro & 42.28 & 53.29 & 57.21 & 36.80 & 50.07 & 53.67 & 37.47 & 52.94 & 55.18 & 29.18 & 49.44 & 50.00 & 38.68 & 48.68 & 54.08 & 22.05 & 41.23 & 46.23 & 34.41 & 49.28 & 52.73 & 45.47 \\
Qwen2.5 72B & -- & 47.55 & -- & -- & 45.17 & -- & -- & 50.62 & -- & -- & 42.70 & -- & -- & 44.47 & -- & -- & 37.95 & -- & -- & 44.74 & -- & 44.74 \\
\rowcolor{gray!20}
Qwen2.5 32B & -- & 47.89 & -- & -- & 43.73 & -- & -- & 48.45 & -- & -- & 40.71 & -- & -- & 42.17 & -- & -- & 39.25 & -- & -- & 43.70 & -- & 43.70 \\
GPT-4o Mini & 34.36 & 48.89 & 55.70 & 27.70 & 46.63 & 54.00 & 30.73 & 49.05 & 53.61 & 24.95 & 43.72 & 49.44 & 36.84 & 47.50 & 54.21 & 21.03 & 39.25 & 46.78 & 29.27 & 45.84 & 52.29 & 42.47 \\
\rowcolor{gray!20}
Gemini Flash & 36.54 & 52.75 & 54.70 & 29.67 & 46.87 & 51.30 & 31.78 & 50.40 & 51.62 & 23.20 & 46.07 & 49.07 & 32.43 & 46.64 & 51.45 & 16.44 & 36.37 & 42.12 & 28.34 & 46.52 & 50.04 & 41.63 \\
Phi 3.5 Mini & -- & 40.40 & -- & -- & 35.23 & -- & -- & 38.27 & -- & -- & 34.80 & -- & -- & 34.87 & -- & -- & 30.00 & -- & -- & 35.60 & -- & 35.60 \\
\rowcolor{gray!20}
Aya Expanse 8B & -- & 40.17 & -- & -- & 36.13 & -- & -- & 39.42 & -- & -- & 34.18 & -- & -- & 36.32 & -- & -- & 26.71 & -- & -- & 35.49 & -- & 35.49 \\
Qwen2.5 7B & -- & 38.39 & -- & -- & 36.50 & -- & -- & 38.78 & -- & -- & 34.23 & -- & -- & 34.01 & -- & -- & 29.04 & -- & -- & 35.16 & -- & 35.16 \\
\rowcolor{gray!20}
InternLM2.5 20B & -- & 37.01 & -- & -- & 34.13 & -- & -- & 36.59 & -- & -- & 31.17 & -- & -- & 32.83 & -- & -- & 27.53 & -- & -- & 33.21 & -- & 33.21 \\
Llama 3.2 11B Vision & -- & 36.44 & -- & -- & 32.77 & -- & -- & 35.75 & -- & -- & 30.00 & -- & -- & 33.68 & -- & -- & 27.40 & -- & -- & 32.67 & -- & 32.67 \\
\rowcolor{gray!20}
InternVL2.5 38B & 23.72 & 41.21 & 37.62 & 18.63 & 38.80 & 37.03 & 20.51 & 41.55 & 39.96 & 23.72 & 33.32 & 38.72 & 24.08 & 35.46 & 39.67 & 15.96 & 32.47 & 33.49 & 21.10 & 37.14 & 37.75 & 32.00 \\
InternVL2.5 78B & 19.33 & 40.84 & 36.28 & 17.63 & 37.73 & 37.10 & 19.16 & 41.57 & 38.23 & 19.64 & 37.50 & 36.58 & 22.89 & 35.66 & 42.57 & 14.86 & 33.22 & 35.34 & 18.92 & 37.75 & 37.68 & 31.45 \\
\rowcolor{gray!20}
Qwen2 VL 72B & 20.67 & 40.81 & 41.01 & 17.37 & 37.03 & 42.13 & 18.23 & 40.02 & 42.10 & 14.08 & 36.02 & 37.60 & 23.42 & 36.12 & 41.91 & 10.62 & 29.38 & 35.14 & 17.40 & 36.56 & 39.98 & 31.31 \\
InternLM2.5 7B & -- & 34.33 & -- & -- & 32.30 & -- & -- & 34.62 & -- & -- & 31.17 & -- & -- & 29.93 & -- & -- & 23.49 & -- & -- & 30.97 & -- & 30.97 \\
\rowcolor{gray!20}
Qwen2.5 3B & -- & 32.75 & -- & -- & 28.90 & -- & -- & 33.05 & -- & -- & 28.47 & -- & -- & 26.58 & -- & -- & 22.81 & -- & -- & 28.76 & -- & 28.76 \\
InternVL2.5 26B & 11.91 & 39.97 & 34.43 & 12.63 & 36.10 & 34.07 & 13.76 & 38.92 & 34.00 & 13.11 & 34.18 & 28.98 & 15.33 & 34.01 & 36.38 & 9.38 & 29.59 & 27.95 & 12.69 & 35.46 & 32.64 & 26.93 \\
\rowcolor{gray!20}
Qwen2 VL 7B & 14.09 & 32.82 & 38.09 & 14.27 & 29.53 & 37.17 & 12.72 & 33.12 & 37.43 & 17.09 & 28.32 & 35.97 & 17.17 & 29.28 & 35.46 & 9.38 & 20.55 & 30.96 & 14.12 & 28.94 & 35.85 & 26.30 \\
MiniCPM V 2.6 & 18.49 & 34.70 & 36.28 & 13.60 & 30.47 & 34.60 & 15.88 & 33.76 & 34.96 & 18.67 & 29.03 & 34.34 & 17.50 & 30.20 & 36.84 & 9.93 & 18.42 & 24.52 & 15.68 & 29.43 & 33.59 & 26.23 \\
\rowcolor{gray!20}
Centurio Qwen & 14.87 & 31.38 & 32.05 & 14.47 & 29.23 & 29.97 & 15.07 & 31.57 & 34.76 & 16.38 & 27.40 & 35.77 & 18.62 & 27.30 & 36.32 & 13.01 & 20.41 & 32.60 & 15.40 & 27.88 & 33.58 & 25.62 \\
Phi 3.5 Vision & 12.08 & 36.64 & 35.03 & 12.43 & 32.10 & 35.23 & 10.09 & 33.36 & 32.30 & 13.78 & 29.74 & 29.80 & 16.97 & 31.97 & 33.42 & 11.99 & 25.75 & 26.78 & 12.89 & 31.59 & 32.09 & 25.53 \\
\rowcolor{gray!20}
InternVL2.5 8B & 6.81 & 36.28 & 29.97 & 6.80 & 31.33 & 29.13 & 9.07 & 33.72 & 30.49 & 6.58 & 29.74 & 30.36 & 12.11 & 30.53 & 30.26 & 2.53 & 22.67 & 20.96 & 7.32 & 30.71 & 28.53 & 22.19 \\
InternVL2.5 4B & 5.44 & 35.81 & 27.89 & 5.40 & 33.07 & 27.80 & 5.97 & 35.71 & 28.08 & 7.14 & 34.29 & 27.24 & 9.01 & 28.62 & 29.54 & 4.79 & 25.68 & 23.63 & 6.29 & 32.20 & 27.36 & 21.95 \\
\rowcolor{gray!20}
Qwen2.5 1.5B & -- & 24.03 & -- & -- & 20.77 & -- & -- & 26.66 & -- & -- & 20.87 & -- & -- & 21.45 & -- & -- & 16.23 & -- & -- & 21.67 & -- & 21.67 \\
InternLM2.5 1.8B & -- & 23.56 & -- & -- & 22.30 & -- & -- & 22.94 & -- & -- & 18.52 & -- & -- & 21.78 & -- & -- & 14.66 & -- & -- & 20.63 & -- & 20.63 \\
\rowcolor{gray!20}
Qwen2 VL 2B & 11.41 & 23.29 & 31.95 & 11.57 & 20.03 & 28.90 & 12.48 & 20.97 & 29.00 & 14.18 & 20.51 & 28.16 & 16.32 & 18.29 & 29.47 & 11.92 & 13.63 & 25.96 & 12.98 & 19.45 & 28.91 & 20.45 \\
InternVL2.5 1B & 9.87 & 24.09 & 16.51 & 8.50 & 20.43 & 16.83 & 9.78 & 21.28 & 18.50 & 11.22 & 20.41 & 16.07 & 12.83 & 16.51 & 18.75 & 9.93 & 14.93 & 17.60 & 10.35 & 19.61 & 17.38 & 15.78 \\
\rowcolor{gray!20}
InternVL2.5 2B & 5.30 & 23.26 & 18.72 & 4.80 & 19.50 & 21.90 & 4.47 & 22.26 & 20.58 & 7.30 & 21.48 & 19.95 & 9.34 & 21.38 & 20.72 & 5.68 & 15.96 & 18.77 & 6.15 & 20.64 & 20.11 & 15.63 \\
Centurio Aya & 4.80 & 29.33 & 5.94 & 5.30 & 25.50 & 7.53 & 2.94 & 28.85 & 5.02 & 7.50 & 24.23 & 8.47 & 4.28 & 24.21 & 4.21 & 4.45 & 19.38 & 5.89 & 4.88 & 25.25 & 6.18 & 12.10 \\
\rowcolor{gray!20}
Qwen2.5 0.5B & -- & 13.96 & -- & -- & 11.77 & -- & -- & 14.40 & -- & -- & 11.43 & -- & -- & 8.29 & -- & -- & 8.70 & -- & -- & 11.42 & -- & 11.42 \\
\midrule
Average X-Large LVLMs & 20.00 & 40.83 & 38.64 & 17.50 & 37.38 & 39.62 & 18.70 & 40.80 & 40.16 & 16.86 & 36.76 & 37.09 & 23.16 & 35.89 & 42.24 & 12.74 & 31.30 & 35.24 & 18.16 & 37.16 & 38.83 & 31.38 \\
\rowcolor{gray!20}
Average Large LVLMs & 17.81 & 40.59 & 36.02 & 15.63 & 37.45 & 35.55 & 17.14 & 40.24 & 36.98 & 18.42 & 33.75 & 33.85 & 19.70 & 34.74 & 38.03 & 12.67 & 31.03 & 30.72 & 16.90 & 36.30 & 35.20 & 29.46 \\
Average Medium LVLMs & 11.81 & 33.49 & 28.47 & 10.89 & 29.80 & 27.68 & 11.14 & 32.79 & 28.53 & 13.24 & 28.12 & 28.98 & 13.94 & 29.20 & 28.62 & 7.86 & 21.47 & 22.99 & 11.48 & 29.15 & 27.55 & 24.18 \\
\rowcolor{gray!20}
Average Small LVLMs & 8.82 & 28.62 & 26.02 & 8.54 & 25.03 & 26.13 & 8.56 & 26.72 & 25.69 & 10.72 & 25.29 & 24.24 & 12.89 & 23.35 & 26.38 & 8.86 & 19.19 & 22.55 & 9.73 & 24.70 & 25.17 & 19.87 \\
Average LVLMs & 12.77 & 33.79 & 30.13 & 11.67 & 30.24 & 29.96 & 12.15 & 32.83 & 30.39 & 13.60 & 29.08 & 29.14 & 15.70 & 28.88 & 31.11 & 9.60 & 23.30 & 25.68 & 12.58 & 29.69 & 29.40 & 24.41 \\
\rowcolor{gray!20}
Average X-Large LLMs & -- & 47.55 & -- & -- & 45.17 & -- & -- & 50.62 & -- & -- & 42.70 & -- & -- & 44.47 & -- & -- & 37.95 & -- & -- & 44.74 & -- & 44.74 \\
Average Large LLMs & -- & 42.45 & -- & -- & 38.93 & -- & -- & 42.52 & -- & -- & 35.94 & -- & -- & 37.50 & -- & -- & 33.39 & -- & -- & 38.46 & -- & 38.46 \\
\rowcolor{gray!20}
Average Medium LLMs & -- & 37.63 & -- & -- & 34.98 & -- & -- & 37.61 & -- & -- & 33.19 & -- & -- & 33.42 & -- & -- & 26.41 & -- & -- & 33.87 & -- & 33.87 \\
Average Small LLMs & -- & 26.94 & -- & -- & 23.79 & -- & -- & 27.06 & -- & -- & 22.82 & -- & -- & 22.59 & -- & -- & 18.48 & -- & -- & 23.62 & -- & 23.62 \\
\rowcolor{gray!20}
Average LLMs & -- & 34.55 & -- & -- & 31.54 & -- & -- & 34.89 & -- & -- & 29.84 & -- & -- & 30.25 & -- & -- & 25.12 & -- & -- & 31.03 & -- & 31.03 \\
Average X-Large & 20.00 & 43.07 & 38.64 & 17.50 & 39.98 & 39.62 & 18.70 & 44.07 & 40.16 & 16.86 & 38.74 & 37.09 & 23.16 & 38.75 & 42.24 & 12.74 & 33.52 & 35.24 & 18.16 & 39.68 & 38.83 & 35.83 \\
\rowcolor{gray!20}
Average Large & 17.81 & 41.52 & 36.02 & 15.63 & 38.19 & 35.55 & 17.14 & 41.38 & 36.98 & 18.42 & 34.84 & 33.85 & 19.70 & 36.12 & 38.03 & 12.67 & 32.21 & 30.72 & 16.90 & 37.38 & 35.20 & 33.96 \\
Average Medium & 11.81 & 34.87 & 28.47 & 10.89 & 31.53 & 27.68 & 11.14 & 34.40 & 28.53 & 13.24 & 29.81 & 28.98 & 13.94 & 30.61 & 28.62 & 7.86 & 23.12 & 22.99 & 11.48 & 30.72 & 27.55 & 27.41 \\
\rowcolor{gray!20}
Average Small & 8.82 & 27.78 & 26.02 & 8.54 & 24.41 & 26.13 & 8.56 & 26.89 & 25.69 & 10.72 & 24.05 & 24.24 & 12.89 & 22.97 & 26.38 & 8.86 & 18.84 & 22.55 & 9.73 & 24.16 & 25.17 & 21.74 \\
Average Open & 12.77 & 34.11 & 30.13 & 11.67 & 30.79 & 29.96 & 12.15 & 33.70 & 30.39 & 13.60 & 29.40 & 29.14 & 15.70 & 29.46 & 31.11 & 9.60 & 24.07 & 25.68 & 12.58 & 30.26 & 29.40 & 27.21 \\
\rowcolor{gray!20}
Average Proprietary & 40.64 & 53.67 & 56.08 & 33.51 & 50.77 & 52.78 & 36.85 & 54.25 & 54.60 & 27.65 & 48.82 & 50.04 & 38.76 & 51.47 & 54.07 & 22.66 & 43.57 & 46.26 & 33.35 & 50.43 & 52.31 & 45.36 \\
Average & 20.11 & 37.27 & 36.96 & 17.42 & 34.01 & 35.96 & 18.65 & 37.02 & 36.76 & 17.30 & 32.53 & 34.64 & 21.77 & 33.01 & 37.15 & 13.04 & 27.22 & 31.10 & 18.05 & 33.51 & 35.43 & 30.14 \\
\bottomrule
\end{tabular}

==> tables/ckqa_naming_acc_scores.tex <==
\begin{tabular}{lrrrrrrr}
\toprule
region & West EU \& North America & East EU & Asia \& Pacific & Latin-America \& Caribbean & Arab & Subsaharian Africa & Average \\
model &  &  &  &  &  &  &  \\
\midrule
\rowcolor{gray!20}
GPT-4o & 37.79 & 32.57 & 37.68 & 30.15 & 38.03 & 28.42 & 34.11 \\
Claude 3.5 Sonnet & 40.27 & 33.63 & 39.29 & 25.71 & 38.16 & 24.25 & 33.55 \\
\rowcolor{gray!20}
GPT-4o Mini & 34.46 & 28.73 & 33.08 & 23.67 & 34.87 & 25.89 & 30.12 \\
Centurio Qwen & 18.69 & 19.10 & 21.97 & 18.67 & 25.46 & 15.96 & 19.98 \\
\rowcolor{gray!20}
Gemini Pro & 16.91 & 15.60 & 16.71 & 11.13 & 17.30 & 10.55 & 14.70 \\
Gemini Flash & 15.77 & 16.27 & 14.87 & 11.60 & 14.61 & 11.30 & 14.07 \\
\rowcolor{gray!20}
InternVL2.5 38B & 14.06 & 12.60 & 16.24 & 10.71 & 21.12 & 8.36 & 13.85 \\
Phi 3.5 Vision & 15.17 & 13.67 & 13.54 & 12.45 & 14.28 & 10.75 & 13.31 \\
\rowcolor{gray!20}
InternVL2.5 78B & 12.08 & 14.73 & 14.89 & 7.35 & 15.72 & 7.53 & 12.05 \\
InternVL2.5 26B & 11.51 & 10.50 & 13.16 & 7.65 & 14.34 & 7.74 & 10.82 \\
\rowcolor{gray!20}
InternVL2.5 1B & 10.20 & 9.43 & 10.42 & 10.71 & 14.80 & 8.22 & 10.63 \\
Qwen2 VL 72B & 11.04 & 10.07 & 9.96 & 7.40 & 11.45 & 8.56 & 9.75 \\
\rowcolor{gray!20}
MiniCPM V 2.6 & 8.89 & 8.60 & 11.42 & 4.74 & 10.99 & 9.79 & 9.07 \\
Centurio Aya & 6.95 & 6.57 & 6.06 & 8.78 & 5.20 & 7.40 & 6.83 \\
\rowcolor{gray!20}
InternVL2.5 2B & 6.31 & 6.80 & 6.17 & 7.14 & 8.49 & 3.08 & 6.33 \\
InternVL2.5 4B & 6.28 & 5.47 & 5.07 & 6.02 & 9.28 & 5.00 & 6.19 \\
\rowcolor{gray!20}
InternVL2.5 8B & 6.51 & 5.30 & 4.54 & 6.48 & 9.28 & 3.77 & 5.98 \\
Qwen2 VL 2B & 5.40 & 4.27 & 7.35 & 3.62 & 5.53 & 3.63 & 4.97 \\
\rowcolor{gray!20}
Qwen2 VL 7B & 5.27 & 5.63 & 4.78 & 4.03 & 6.32 & 3.70 & 4.96 \\
\midrule
Average X-Large LVLMs & 11.56 & 12.40 & 12.42 & 7.38 & 13.58 & 8.04 & 10.90 \\
\rowcolor{gray!20}
Average Large LVLMs & 12.78 & 11.55 & 14.70 & 9.18 & 17.73 & 8.05 & 12.34 \\
Average Medium LVLMs & 9.26 & 9.04 & 9.75 & 8.54 & 11.45 & 8.12 & 9.36 \\
\rowcolor{gray!20}
Average Small LVLMs & 8.67 & 7.93 & 8.51 & 7.99 & 10.48 & 6.14 & 8.29 \\
Average LVLMs & 9.88 & 9.48 & 10.40 & 8.27 & 12.30 & 7.39 & 9.62 \\
\rowcolor{gray!20}
Average X-Large & 11.56 & 12.40 & 12.42 & 7.38 & 13.58 & 8.04 & 10.90 \\
Average Large & 12.78 & 11.55 & 14.70 & 9.18 & 17.73 & 8.05 & 12.34 \\
\rowcolor{gray!20}
Average Medium & 9.26 & 9.04 & 9.75 & 8.54 & 11.45 & 8.12 & 9.36 \\
Average Small & 8.67 & 7.93 & 8.51 & 7.99 & 10.48 & 6.14 & 8.29 \\
\rowcolor{gray!20}
Average Open & 9.88 & 9.48 & 10.40 & 8.27 & 12.30 & 7.39 & 9.62 \\
Average Proprietary & 29.04 & 25.36 & 28.33 & 20.45 & 28.59 & 20.08 & 25.31 \\
\rowcolor{gray!20}
Average & 14.92 & 13.66 & 15.12 & 11.47 & 16.59 & 10.73 & 13.75 \\
\bottomrule
\end{tabular}

==> tables/coqa_countries_acc_scores.tex <==
\begin{tabular}{llrllrllrllrllrllrllrlr}
\toprule
region & \multicolumn{3}{r}{West EU \& North America} & \multicolumn{3}{r}{East EU} & \multicolumn{3}{r}{Asia \& Pacific} & \multicolumn{3}{r}{Latin-America \& Caribbean} & \multicolumn{3}{r}{Arab} & \multicolumn{3}{r}{Subsaharian Africa} & \multicolumn{4}{r}{Average} \\
combination & I & T & I+T & I & T & I+T & I & T & I+T & I & T & I+T & I & T & I+T & I & T & I+T & I & T & I+T & Avg \\
model &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
\midrule
\rowcolor{gray!20}
Claude 3.5 Sonnet & 79.23 & 96.72 & 95.63 & 82.35 & 97.65 & 96.47 & 76.62 & 97.84 & 95.67 & 70.21 & 98.94 & 100.00 & 76.47 & 97.65 & 96.47 & 83.82 & 97.06 & 91.18 & 78.12 & 97.64 & 95.90 & 90.55 \\
GPT-4o & 93.44 & 95.08 & 96.17 & 94.71 & 98.24 & 98.24 & 93.51 & 97.40 & 98.27 & 97.87 & 98.94 & 98.94 & 95.29 & 95.29 & 98.82 & 95.59 & 97.06 & 100.00 & 95.07 & 97.00 & 98.41 & 96.83 \\
\rowcolor{gray!20}
InternVL2.5 78B & 83.06 & 94.54 & 97.81 & 80.59 & 95.88 & 97.65 & 83.12 & 93.51 & 96.54 & 81.91 & 98.94 & 98.94 & 90.59 & 97.65 & 97.65 & 83.82 & 97.06 & 98.53 & 83.85 & 96.26 & 97.85 & 92.65 \\
Qwen2.5 72B & -- & 93.44 & -- & -- & 96.47 & -- & -- & 94.81 & -- & -- & 98.94 & -- & -- & 97.65 & -- & -- & 94.12 & -- & -- & 95.90 & -- & 95.90 \\
\rowcolor{gray!20}
GPT-4o Mini & 89.07 & 93.99 & 95.63 & 90.00 & 95.29 & 97.65 & 90.48 & 93.51 & 96.97 & 90.43 & 95.74 & 100.00 & 94.12 & 88.24 & 97.65 & 91.18 & 95.59 & 98.53 & 90.88 & 93.73 & 97.74 & 94.11 \\
Qwen2.5 32B & -- & 91.26 & -- & -- & 93.53 & -- & -- & 91.77 & -- & -- & 94.68 & -- & -- & 95.29 & -- & -- & 92.65 & -- & -- & 93.20 & -- & 93.20 \\
\rowcolor{gray!20}
InternVL2.5 38B & 78.69 & 91.80 & 92.35 & 77.06 & 91.18 & 92.94 & 77.49 & 93.07 & 93.94 & 79.79 & 95.74 & 96.81 & 84.71 & 94.12 & 95.29 & 88.24 & 92.65 & 98.53 & 80.99 & 93.09 & 94.98 & 89.69 \\
Qwen2 VL 72B & 87.98 & 87.43 & 95.08 & 94.12 & 90.59 & 96.47 & 90.04 & 90.04 & 97.84 & 91.49 & 97.87 & 98.94 & 92.94 & 89.41 & 98.82 & 91.18 & 97.06 & 98.53 & 91.29 & 92.07 & 97.61 & 93.66 \\
\rowcolor{gray!20}
Gemini Flash & 90.56 & 89.01 & 97.27 & 90.59 & 88.82 & 97.06 & 91.77 & 90.48 & 98.70 & 90.43 & 93.62 & 97.87 & 90.59 & 88.24 & 97.65 & 88.24 & 95.59 & 97.06 & 90.36 & 90.96 & 97.60 & 92.97 \\
InternVL2.5 26B & 78.14 & 87.98 & 92.90 & 78.24 & 88.24 & 94.71 & 76.19 & 90.48 & 93.94 & 80.85 & 94.68 & 94.68 & 81.18 & 91.76 & 91.76 & 80.88 & 91.18 & 95.59 & 79.25 & 90.72 & 93.93 & 87.96 \\
\rowcolor{gray!20}
Qwen2.5 7B & -- & 86.34 & -- & -- & 88.24 & -- & -- & 85.28 & -- & -- & 95.74 & -- & -- & 90.59 & -- & -- & 94.12 & -- & -- & 90.05 & -- & 90.05 \\
Aya Expanse 8B & -- & 87.43 & -- & -- & 88.24 & -- & -- & 90.04 & -- & -- & 93.62 & -- & -- & 88.24 & -- & -- & 89.71 & -- & -- & 89.54 & -- & 89.54 \\
\rowcolor{gray!20}
InternLM2.5 20B & -- & 86.89 & -- & -- & 87.06 & -- & -- & 90.91 & -- & -- & 90.43 & -- & -- & 85.88 & -- & -- & 89.71 & -- & -- & 88.48 & -- & 88.48 \\
MiniCPM V 2.6 & 81.97 & 84.70 & 90.16 & 81.18 & 86.47 & 92.94 & 78.79 & 87.45 & 92.21 & 86.17 & 87.23 & 92.55 & 82.35 & 89.41 & 96.47 & 88.24 & 92.65 & 94.12 & 83.12 & 87.98 & 93.08 & 88.06 \\
\rowcolor{gray!20}
Qwen2 VL 7B & 87.43 & 83.61 & 90.71 & 82.35 & 85.29 & 92.94 & 87.01 & 84.85 & 94.37 & 91.49 & 88.30 & 94.68 & 84.71 & 88.24 & 96.47 & 92.65 & 94.12 & 97.06 & 87.61 & 87.40 & 94.37 & 89.79 \\
Qwen2.5 3B & -- & 81.42 & -- & -- & 85.88 & -- & -- & 84.85 & -- & -- & 92.55 & -- & -- & 88.24 & -- & -- & 86.76 & -- & -- & 86.62 & -- & 86.62 \\
\rowcolor{gray!20}
InternLM2.5 7B & -- & 83.61 & -- & -- & 85.88 & -- & -- & 85.71 & -- & -- & 90.43 & -- & -- & 77.65 & -- & -- & 88.24 & -- & -- & 85.25 & -- & 85.25 \\
Centurio Qwen & 78.69 & 82.51 & 89.07 & 78.82 & 82.94 & 89.41 & 78.79 & 84.42 & 92.64 & 76.60 & 85.11 & 91.49 & 80.00 & 83.53 & 88.24 & 79.41 & 91.18 & 92.65 & 78.72 & 84.95 & 90.58 & 84.75 \\
\rowcolor{gray!20}
Centurio Aya & 65.57 & 83.61 & 85.79 & 72.35 & 81.76 & 85.88 & 75.76 & 85.71 & 88.31 & 74.47 & 87.23 & 82.98 & 70.59 & 80.00 & 89.41 & 66.18 & 89.71 & 89.71 & 70.82 & 84.67 & 87.01 & 80.83 \\
InternVL2.5 8B & 68.31 & 82.51 & 88.52 & 70.59 & 84.71 & 90.00 & 75.32 & 86.58 & 91.34 & 75.53 & 87.23 & 94.68 & 76.47 & 83.53 & 90.59 & 82.35 & 82.35 & 89.71 & 74.76 & 84.49 & 90.81 & 83.35 \\
\rowcolor{gray!20}
Phi 3.5 Mini & -- & 80.87 & -- & -- & 82.94 & -- & -- & 83.98 & -- & -- & 84.04 & -- & -- & 82.35 & -- & -- & 88.24 & -- & -- & 83.74 & -- & 83.74 \\
InternVL2.5 4B & 68.85 & 77.05 & 89.62 & 72.35 & 82.94 & 89.41 & 71.43 & 86.15 & 90.48 & 76.60 & 87.23 & 89.36 & 72.94 & 81.18 & 84.71 & 76.47 & 82.35 & 97.06 & 73.11 & 82.82 & 90.11 & 82.01 \\
\rowcolor{gray!20}
Phi 3.5 Vision & 72.13 & 79.78 & 86.89 & 68.82 & 82.94 & 92.35 & 69.70 & 81.82 & 89.61 & 74.47 & 91.49 & 91.49 & 81.18 & 77.65 & 90.59 & 76.47 & 82.35 & 95.59 & 73.79 & 82.67 & 91.09 & 82.52 \\
Qwen2.5 1.5B & -- & 78.69 & -- & -- & 81.18 & -- & -- & 82.68 & -- & -- & 82.98 & -- & -- & 75.29 & -- & -- & 80.88 & -- & -- & 80.28 & -- & 80.28 \\
\rowcolor{gray!20}
Qwen2 VL 2B & 83.06 & 74.32 & 87.43 & 84.71 & 77.06 & 87.65 & 83.55 & 80.95 & 90.48 & 92.55 & 81.91 & 94.68 & 83.53 & 76.47 & 91.76 & 89.71 & 80.88 & 94.12 & 86.18 & 78.60 & 91.02 & 85.27 \\
Qwen2.5 0.5B & -- & 65.03 & -- & -- & 68.82 & -- & -- & 72.29 & -- & -- & 75.53 & -- & -- & 69.41 & -- & -- & 77.94 & -- & -- & 71.51 & -- & 71.51 \\
\rowcolor{gray!20}
InternVL2.5 1B & 61.20 & 66.12 & 73.77 & 59.41 & 65.88 & 73.53 & 62.34 & 75.76 & 77.06 & 67.02 & 74.47 & 76.60 & 56.47 & 63.53 & 75.29 & 55.88 & 72.06 & 70.59 & 60.39 & 69.64 & 74.47 & 68.17 \\
InternLM2.5 1.8B & -- & 63.39 & -- & -- & 66.47 & -- & -- & 71.00 & -- & -- & 67.02 & -- & -- & 58.82 & -- & -- & 64.71 & -- & -- & 65.23 & -- & 65.23 \\
\rowcolor{gray!20}
InternVL2.5 2B & 62.84 & 65.57 & 74.32 & 61.76 & 64.71 & 72.35 & 61.04 & 68.40 & 80.95 & 67.02 & 68.09 & 80.85 & 67.06 & 55.29 & 74.12 & 73.53 & 63.24 & 77.94 & 65.54 & 64.22 & 76.76 & 68.84 \\
Gemini Pro & 76.67 & 43.17 & 92.70 & 75.88 & 39.41 & 92.94 & 78.79 & 34.20 & 92.64 & 78.72 & 39.36 & 93.62 & 78.82 & 35.29 & 91.76 & 82.35 & 19.12 & 94.12 & 78.54 & 35.09 & 92.96 & 68.86 \\
\midrule
Average X-Large LVLMs & 85.52 & 90.98 & 96.45 & 87.35 & 93.24 & 97.06 & 86.58 & 91.77 & 97.19 & 86.70 & 98.40 & 98.94 & 91.76 & 93.53 & 98.24 & 87.50 & 97.06 & 98.53 & 87.57 & 94.16 & 97.73 & 93.16 \\
\rowcolor{gray!20}
Average Large LVLMs & 78.42 & 89.89 & 92.62 & 77.65 & 89.71 & 93.82 & 76.84 & 91.77 & 93.94 & 80.32 & 95.21 & 95.74 & 82.94 & 92.94 & 93.53 & 84.56 & 91.91 & 97.06 & 80.12 & 91.90 & 94.46 & 88.82 \\
Average Medium LVLMs & 76.39 & 83.39 & 88.85 & 77.06 & 84.24 & 90.24 & 79.13 & 85.80 & 91.77 & 80.85 & 87.02 & 91.28 & 78.82 & 84.94 & 92.24 & 81.76 & 90.00 & 92.65 & 79.01 & 85.90 & 91.17 & 85.36 \\
\rowcolor{gray!20}
Average Small LVLMs & 69.62 & 72.57 & 82.40 & 69.41 & 74.71 & 83.06 & 69.61 & 78.61 & 85.71 & 75.53 & 80.64 & 86.60 & 72.24 & 70.82 & 83.29 & 74.41 & 76.18 & 87.06 & 71.80 & 75.59 & 84.69 & 77.36 \\
Average LVLMs & 75.57 & 81.54 & 88.17 & 75.88 & 82.90 & 89.16 & 76.47 & 84.94 & 90.69 & 79.71 & 87.54 & 91.34 & 78.91 & 82.27 & 90.08 & 80.36 & 86.34 & 92.12 & 77.82 & 84.26 & 90.26 & 84.11 \\
\rowcolor{gray!20}
Average X-Large LLMs & -- & 93.44 & -- & -- & 96.47 & -- & -- & 94.81 & -- & -- & 98.94 & -- & -- & 97.65 & -- & -- & 94.12 & -- & -- & 95.90 & -- & 95.90 \\
Average Large LLMs & -- & 89.07 & -- & -- & 90.29 & -- & -- & 91.34 & -- & -- & 92.55 & -- & -- & 90.59 & -- & -- & 91.18 & -- & -- & 90.84 & -- & 90.84 \\
\rowcolor{gray!20}
Average Medium LLMs & -- & 85.79 & -- & -- & 87.45 & -- & -- & 87.01 & -- & -- & 93.26 & -- & -- & 85.49 & -- & -- & 90.69 & -- & -- & 88.28 & -- & 88.28 \\
Average Small LLMs & -- & 73.88 & -- & -- & 77.06 & -- & -- & 78.96 & -- & -- & 80.43 & -- & -- & 74.82 & -- & -- & 79.71 & -- & -- & 77.48 & -- & 77.48 \\
\rowcolor{gray!20}
Average LLMs & -- & 81.67 & -- & -- & 84.06 & -- & -- & 84.85 & -- & -- & 87.81 & -- & -- & 82.67 & -- & -- & 86.10 & -- & -- & 84.53 & -- & 84.53 \\
Average X-Large & 85.52 & 91.80 & 96.45 & 87.35 & 94.31 & 97.06 & 86.58 & 92.78 & 97.19 & 86.70 & 98.58 & 98.94 & 91.76 & 94.90 & 98.24 & 87.50 & 96.08 & 98.53 & 87.57 & 94.74 & 97.73 & 94.07 \\
\rowcolor{gray!20}
Average Large & 78.42 & 89.48 & 92.62 & 77.65 & 90.00 & 93.82 & 76.84 & 91.56 & 93.94 & 80.32 & 93.88 & 95.74 & 82.94 & 91.76 & 93.53 & 84.56 & 91.54 & 97.06 & 80.12 & 91.37 & 94.46 & 89.83 \\
Average Medium & 76.39 & 84.29 & 88.85 & 77.06 & 85.44 & 90.24 & 79.13 & 86.26 & 91.77 & 80.85 & 89.36 & 91.28 & 78.82 & 85.15 & 92.24 & 81.76 & 90.26 & 92.65 & 79.01 & 86.79 & 91.17 & 86.45 \\
\rowcolor{gray!20}
Average Small & 69.62 & 73.22 & 82.40 & 69.41 & 75.88 & 83.06 & 69.61 & 78.79 & 85.71 & 75.53 & 80.53 & 86.60 & 72.24 & 72.82 & 83.29 & 74.41 & 77.94 & 87.06 & 71.80 & 76.53 & 84.69 & 77.42 \\
Average Open & 75.57 & 81.60 & 88.17 & 75.88 & 83.41 & 89.16 & 76.47 & 84.90 & 90.69 & 79.71 & 87.66 & 91.34 & 78.91 & 82.45 & 90.08 & 80.36 & 86.24 & 92.12 & 77.82 & 84.38 & 90.26 & 84.29 \\
\rowcolor{gray!20}
Average Proprietary & 85.79 & 83.59 & 95.48 & 86.71 & 83.88 & 96.47 & 86.23 & 82.68 & 96.45 & 85.53 & 85.32 & 98.09 & 87.06 & 80.94 & 96.47 & 88.24 & 80.88 & 96.18 & 86.59 & 82.88 & 96.52 & 88.66 \\
Average & 78.26 & 81.93 & 90.10 & 78.73 & 83.49 & 91.08 & 79.04 & 84.53 & 92.21 & 81.24 & 87.27 & 93.11 & 81.05 & 82.20 & 91.76 & 82.43 & 85.34 & 93.19 & 80.13 & 84.13 & 91.91 & 85.02 \\
\bottomrule
\end{tabular}

==> tables/coqa_regions_acc_scores.tex <==
\begin{tabular}{llrllrllrllrllrllrllrlr}
\toprule
region & \multicolumn{3}{r}{West EU \& North America} & \multicolumn{3}{r}{East EU} & \multicolumn{3}{r}{Asia \& Pacific} & \multicolumn{3}{r}{Latin-America \& Caribbean} & \multicolumn{3}{r}{Arab} & \multicolumn{3}{r}{Subsaharian Africa} & \multicolumn{4}{r}{Average} \\
combination & I & T & I+T & I & T & I+T & I & T & I+T & I & T & I+T & I & T & I+T & I & T & I+T & I & T & I+T & Avg \\
model &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
\midrule
\rowcolor{gray!20}
GPT-4o & 82.50 & 83.75 & 85.00 & 85.89 & 90.18 & 88.34 & 94.37 & 96.54 & 97.40 & 93.68 & 92.63 & 92.63 & 88.00 & 88.00 & 92.00 & 91.30 & 91.30 & 94.20 & 89.29 & 90.40 & 91.60 & 90.43 \\
Claude 3.5 Sonnet & 72.50 & 83.75 & 81.25 & 76.69 & 85.89 & 82.21 & 87.88 & 95.67 & 95.67 & 83.16 & 89.47 & 87.37 & 84.00 & 90.67 & 90.67 & 82.61 & 89.86 & 88.41 & 81.14 & 89.22 & 87.60 & 85.98 \\
\rowcolor{gray!20}
InternVL2.5 78B & 77.50 & 80.00 & 86.88 & 83.44 & 82.21 & 88.96 & 94.37 & 94.81 & 96.97 & 88.42 & 92.63 & 92.63 & 88.00 & 90.67 & 92.00 & 92.75 & 91.30 & 92.75 & 87.41 & 88.60 & 91.70 & 89.24 \\
Qwen2.5 72B & -- & 81.25 & -- & -- & 84.05 & -- & -- & 96.10 & -- & -- & 89.47 & -- & -- & 86.67 & -- & -- & 89.86 & -- & -- & 87.90 & -- & 87.90 \\
\rowcolor{gray!20}
GPT-4o Mini & 76.25 & 82.50 & 86.25 & 84.66 & 82.21 & 84.66 & 94.37 & 95.67 & 96.54 & 87.37 & 90.53 & 90.53 & 85.33 & 86.67 & 86.67 & 91.30 & 89.86 & 92.75 & 86.55 & 87.90 & 89.57 & 88.01 \\
InternVL2.5 38B & 81.25 & 81.25 & 84.38 & 85.89 & 84.66 & 85.28 & 90.04 & 95.24 & 92.64 & 86.32 & 86.32 & 92.63 & 89.33 & 90.67 & 92.00 & 89.86 & 86.96 & 91.30 & 87.11 & 87.51 & 89.70 & 88.11 \\
\rowcolor{gray!20}
Qwen2 VL 72B & 79.38 & 80.62 & 81.25 & 88.34 & 84.66 & 88.34 & 90.48 & 94.81 & 96.97 & 86.32 & 88.42 & 92.63 & 86.67 & 88.00 & 89.33 & 91.30 & 85.51 & 91.30 & 87.08 & 87.00 & 89.97 & 88.02 \\
Gemini Flash & 82.50 & 78.75 & 78.13 & 85.28 & 80.37 & 84.66 & 87.01 & 91.34 & 94.81 & 85.11 & 87.37 & 90.53 & 89.19 & 86.67 & 90.67 & 89.86 & 91.30 & 91.30 & 86.49 & 85.97 & 88.35 & 86.94 \\
\rowcolor{gray!20}
Qwen2.5 32B & -- & 76.88 & -- & -- & 79.75 & -- & -- & 94.37 & -- & -- & 87.37 & -- & -- & 84.00 & -- & -- & 89.86 & -- & -- & 85.37 & -- & 85.37 \\
Qwen2 VL 7B & 71.25 & 74.38 & 76.25 & 82.82 & 80.37 & 84.05 & 92.64 & 93.51 & 93.51 & 85.26 & 88.42 & 92.63 & 80.00 & 82.67 & 84.00 & 86.96 & 85.51 & 84.06 & 83.16 & 84.14 & 85.75 & 84.35 \\
\rowcolor{gray!20}
MiniCPM V 2.6 & 72.50 & 72.50 & 75.00 & 81.60 & 79.14 & 80.37 & 88.74 & 90.48 & 93.07 & 80.00 & 87.37 & 90.53 & 80.00 & 77.33 & 86.67 & 88.41 & 85.51 & 86.96 & 81.87 & 82.05 & 85.43 & 83.12 \\
InternVL2.5 26B & 77.50 & 74.38 & 80.62 & 87.12 & 75.46 & 87.12 & 91.77 & 91.77 & 96.54 & 88.42 & 84.21 & 93.68 & 84.00 & 85.33 & 88.00 & 91.30 & 79.71 & 86.96 & 86.69 & 81.81 & 88.82 & 85.77 \\
\rowcolor{gray!20}
Phi 3.5 Mini & -- & 74.38 & -- & -- & 72.39 & -- & -- & 88.31 & -- & -- & 83.16 & -- & -- & 81.33 & -- & -- & 86.96 & -- & -- & 81.09 & -- & 81.09 \\
InternLM2.5 7B & -- & 74.38 & -- & -- & 76.69 & -- & -- & 90.48 & -- & -- & 80.00 & -- & -- & 78.67 & -- & -- & 85.51 & -- & -- & 80.95 & -- & 80.95 \\
\rowcolor{gray!20}
Centurio Qwen & 75.63 & 74.38 & 80.00 & 79.75 & 76.69 & 82.82 & 86.58 & 92.64 & 92.21 & 83.16 & 86.32 & 89.47 & 78.67 & 77.33 & 88.00 & 86.96 & 76.81 & 89.86 & 81.79 & 80.69 & 87.06 & 83.18 \\
InternLM2.5 20B & -- & 74.38 & -- & -- & 75.46 & -- & -- & 89.18 & -- & -- & 86.32 & -- & -- & 76.00 & -- & -- & 82.61 & -- & -- & 80.66 & -- & 80.66 \\
\rowcolor{gray!20}
Qwen2.5 7B & -- & 71.88 & -- & -- & 72.39 & -- & -- & 93.51 & -- & -- & 85.26 & -- & -- & 77.33 & -- & -- & 81.16 & -- & -- & 80.26 & -- & 80.26 \\
Aya Expanse 8B & -- & 68.12 & -- & -- & 77.30 & -- & -- & 91.77 & -- & -- & 81.05 & -- & -- & 80.00 & -- & -- & 81.16 & -- & -- & 79.90 & -- & 79.90 \\
\rowcolor{gray!20}
InternVL2.5 8B & 68.12 & 72.50 & 75.63 & 83.44 & 76.07 & 83.44 & 87.88 & 89.61 & 94.37 & 84.21 & 83.16 & 92.63 & 84.00 & 73.33 & 89.33 & 88.41 & 81.16 & 92.75 & 82.68 & 79.31 & 88.03 & 83.34 \\
Centurio Aya & 80.62 & 68.12 & 78.75 & 82.21 & 75.46 & 80.37 & 90.91 & 85.71 & 92.21 & 84.21 & 82.11 & 85.26 & 81.33 & 82.67 & 85.33 & 85.51 & 81.16 & 91.30 & 84.13 & 79.21 & 85.54 & 82.96 \\
\rowcolor{gray!20}
Phi 3.5 Vision & 65.62 & 72.50 & 75.63 & 69.94 & 70.55 & 76.69 & 89.18 & 91.34 & 95.24 & 80.00 & 81.05 & 86.32 & 72.00 & 80.00 & 86.67 & 85.51 & 79.71 & 88.41 & 77.04 & 79.19 & 84.82 & 80.35 \\
InternVL2.5 4B & 66.88 & 66.88 & 76.25 & 84.66 & 75.46 & 84.05 & 87.01 & 86.15 & 93.07 & 83.16 & 78.95 & 87.37 & 80.00 & 82.67 & 86.67 & 86.96 & 84.06 & 89.86 & 81.44 & 79.03 & 86.21 & 82.23 \\
\rowcolor{gray!20}
Qwen2 VL 2B & 77.50 & 72.50 & 78.75 & 84.05 & 64.42 & 84.05 & 91.77 & 82.68 & 92.21 & 88.42 & 81.05 & 86.32 & 84.00 & 70.67 & 89.33 & 88.41 & 79.71 & 91.30 & 85.69 & 75.17 & 86.99 & 82.62 \\
Qwen2.5 3B & -- & 68.75 & -- & -- & 73.01 & -- & -- & 83.12 & -- & -- & 73.68 & -- & -- & 74.67 & -- & -- & 75.36 & -- & -- & 74.76 & -- & 74.76 \\
\rowcolor{gray!20}
Qwen2.5 1.5B & -- & 61.88 & -- & -- & 65.03 & -- & -- & 82.25 & -- & -- & 78.95 & -- & -- & 72.00 & -- & -- & 78.26 & -- & -- & 73.06 & -- & 73.06 \\
Qwen2.5 0.5B & -- & 68.12 & -- & -- & 72.39 & -- & -- & 67.53 & -- & -- & 65.26 & -- & -- & 70.67 & -- & -- & 55.07 & -- & -- & 66.51 & -- & 66.51 \\
\rowcolor{gray!20}
InternLM2.5 1.8B & -- & 56.25 & -- & -- & 65.03 & -- & -- & 65.37 & -- & -- & 60.00 & -- & -- & 66.67 & -- & -- & 66.67 & -- & -- & 63.33 & -- & 63.33 \\
InternVL2.5 2B & 70.62 & 51.88 & 72.50 & 76.69 & 58.28 & 71.78 & 77.92 & 72.29 & 82.68 & 83.16 & 62.11 & 83.16 & 73.33 & 66.67 & 82.67 & 84.06 & 60.87 & 89.86 & 77.63 & 62.02 & 80.44 & 73.36 \\
\rowcolor{gray!20}
InternVL2.5 1B & 63.75 & 58.75 & 66.88 & 62.58 & 60.74 & 74.23 & 64.50 & 61.90 & 80.09 & 77.89 & 57.89 & 87.37 & 62.67 & 68.00 & 82.67 & 75.36 & 59.42 & 82.61 & 67.79 & 61.12 & 78.97 & 69.29 \\
Gemini Pro & 76.25 & 59.38 & 78.13 & 68.10 & 55.21 & 82.21 & 82.25 & 56.28 & 89.61 & 79.79 & 61.05 & 85.11 & 79.73 & 61.33 & 84.00 & 72.46 & 65.22 & 95.65 & 76.43 & 59.75 & 85.78 & 73.99 \\
\midrule
Average X-Large LVLMs & 78.44 & 80.31 & 84.06 & 85.89 & 83.44 & 88.65 & 92.42 & 94.81 & 96.97 & 87.37 & 90.53 & 92.63 & 87.33 & 89.33 & 90.67 & 92.03 & 88.41 & 92.03 & 87.24 & 87.80 & 90.84 & 88.63 \\
\rowcolor{gray!20}
Average Large LVLMs & 79.38 & 77.81 & 82.50 & 86.50 & 80.06 & 86.20 & 90.91 & 93.51 & 94.59 & 87.37 & 85.26 & 93.16 & 86.67 & 88.00 & 90.00 & 90.58 & 83.33 & 89.13 & 86.90 & 84.66 & 89.26 & 86.94 \\
Average Medium LVLMs & 73.62 & 72.38 & 77.12 & 81.96 & 77.55 & 82.21 & 89.35 & 90.39 & 93.07 & 83.37 & 85.47 & 90.11 & 80.80 & 78.67 & 86.67 & 87.25 & 82.03 & 88.99 & 82.73 & 81.08 & 86.36 & 83.39 \\
\rowcolor{gray!20}
Average Small LVLMs & 68.88 & 64.50 & 74.00 & 75.58 & 65.89 & 78.16 & 82.08 & 78.87 & 88.66 & 82.53 & 72.21 & 86.11 & 74.40 & 73.60 & 85.60 & 84.06 & 72.75 & 88.41 & 77.92 & 71.31 & 83.49 & 77.57 \\
Average LVLMs & 73.44 & 71.47 & 77.77 & 80.89 & 74.58 & 82.25 & 87.41 & 87.35 & 92.27 & 84.21 & 81.43 & 89.47 & 80.29 & 79.71 & 87.33 & 87.27 & 79.81 & 89.23 & 82.25 & 79.06 & 86.39 & 82.57 \\
\rowcolor{gray!20}
Average X-Large LLMs & -- & 81.25 & -- & -- & 84.05 & -- & -- & 96.10 & -- & -- & 89.47 & -- & -- & 86.67 & -- & -- & 89.86 & -- & -- & 87.90 & -- & 87.90 \\
Average Large LLMs & -- & 75.62 & -- & -- & 77.61 & -- & -- & 91.77 & -- & -- & 86.84 & -- & -- & 80.00 & -- & -- & 86.23 & -- & -- & 83.02 & -- & 83.02 \\
\rowcolor{gray!20}
Average Medium LLMs & -- & 71.46 & -- & -- & 75.46 & -- & -- & 91.92 & -- & -- & 82.11 & -- & -- & 78.67 & -- & -- & 82.61 & -- & -- & 80.37 & -- & 80.37 \\
Average Small LLMs & -- & 65.88 & -- & -- & 69.57 & -- & -- & 77.32 & -- & -- & 72.21 & -- & -- & 73.07 & -- & -- & 72.46 & -- & -- & 71.75 & -- & 71.75 \\
\rowcolor{gray!20}
Average LLMs & -- & 70.57 & -- & -- & 73.95 & -- & -- & 85.64 & -- & -- & 79.14 & -- & -- & 77.09 & -- & -- & 79.31 & -- & -- & 77.62 & -- & 77.62 \\
Average X-Large & 78.44 & 80.62 & 84.06 & 85.89 & 83.64 & 88.65 & 92.42 & 95.24 & 96.97 & 87.37 & 90.18 & 92.63 & 87.33 & 88.44 & 90.67 & 92.03 & 88.89 & 92.03 & 87.24 & 87.83 & 90.84 & 88.39 \\
\rowcolor{gray!20}
Average Large & 79.38 & 76.72 & 82.50 & 86.50 & 78.83 & 86.20 & 90.91 & 92.64 & 94.59 & 87.37 & 86.05 & 93.16 & 86.67 & 84.00 & 90.00 & 90.58 & 84.78 & 89.13 & 86.90 & 83.84 & 89.26 & 84.98 \\
Average Medium & 73.62 & 72.03 & 77.12 & 81.96 & 76.76 & 82.21 & 89.35 & 90.96 & 93.07 & 83.37 & 84.21 & 90.11 & 80.80 & 78.67 & 86.67 & 87.25 & 82.25 & 88.99 & 82.73 & 80.81 & 86.36 & 82.26 \\
\rowcolor{gray!20}
Average Small & 68.88 & 65.19 & 74.00 & 75.58 & 67.73 & 78.16 & 82.08 & 78.10 & 88.66 & 82.53 & 72.21 & 86.11 & 74.40 & 73.33 & 85.60 & 84.06 & 72.61 & 88.41 & 77.92 & 71.53 & 83.49 & 74.66 \\
Average Open & 73.44 & 71.08 & 77.77 & 80.89 & 74.31 & 82.25 & 87.41 & 86.60 & 92.27 & 84.21 & 80.42 & 89.47 & 80.29 & 78.56 & 87.33 & 87.27 & 79.59 & 89.23 & 82.25 & 78.43 & 86.39 & 80.39 \\
\rowcolor{gray!20}
Average Proprietary & 78.00 & 77.62 & 81.75 & 80.12 & 78.77 & 84.42 & 89.18 & 87.10 & 94.81 & 85.82 & 84.21 & 89.23 & 85.25 & 82.67 & 88.80 & 85.51 & 85.51 & 92.46 & 83.98 & 82.65 & 88.58 & 85.07 \\
Average & 74.64 & 72.17 & 78.82 & 80.69 & 75.05 & 82.82 & 87.88 & 86.68 & 92.94 & 84.63 & 81.05 & 89.41 & 81.59 & 79.24 & 87.72 & 86.80 & 80.58 & 90.08 & 82.71 & 79.13 & 86.96 & 81.17 \\
\bottomrule
\end{tabular}

==> tables/sivqa_acc_scores.tex <==
\begin{tabular}{lrrrrrrrrrrrrrrrrrrrrrrrrrrrr}
\toprule
region & \multicolumn{4}{r}{West EU \& North America} & \multicolumn{4}{r}{Asia \& Pacific} & \multicolumn{4}{r}{Subsaharian Africa} & \multicolumn{4}{r}{Arab} & \multicolumn{4}{r}{East EU} & \multicolumn{4}{r}{Latin-America \& Caribbean} & \multicolumn{4}{r}{Average} \\
hint & N & R & C & B & N & R & C & B & N & R & C & B & N & R & C & B & N & R & C & B & N & R & C & B & N & R & C & B \\
model &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
\midrule
\rowcolor{gray!20}
GPT-4o & 31.58 & 34.39 & 41.05 & 40.70 & 29.89 & 31.37 & 36.63 & 37.68 & 17.38 & 17.63 & 32.49 & 31.74 & 25.70 & 30.53 & 39.19 & 39.95 & 26.80 & 32.56 & 42.94 & 41.79 & 23.17 & 25.77 & 30.26 & 32.39 & 25.44 & 28.17 & 36.59 & 37.08 \\
Gemini Pro & 27.02 & 30.53 & 31.23 & 32.28 & 22.53 & 26.11 & 31.16 & 29.68 & 16.84 & 14.61 & 26.20 & 24.18 & 19.85 & 22.39 & 28.50 & 28.50 & 25.07 & 25.94 & 31.12 & 32.56 & 22.46 & 19.86 & 24.35 & 27.19 & 21.50 & 22.84 & 28.30 & 28.30 \\
\rowcolor{gray!20}
GPT-4o Mini & 23.86 & 25.26 & 30.18 & 29.82 & 21.05 & 21.89 & 26.74 & 26.53 & 9.32 & 10.58 & 16.12 & 15.37 & 17.30 & 19.85 & 25.45 & 25.95 & 19.02 & 19.02 & 28.53 & 28.24 & 16.31 & 17.73 & 23.64 & 22.93 & 17.38 & 18.54 & 24.81 & 24.59 \\
Gemini Flash & 22.81 & 25.96 & 27.02 & 24.91 & 18.95 & 20.21 & 26.11 & 25.89 & 12.91 & 10.83 & 20.40 & 18.89 & 15.27 & 17.56 & 20.36 & 20.61 & 20.17 & 19.31 & 24.78 & 24.50 & 14.66 & 16.55 & 22.22 & 20.57 & 16.85 & 18.00 & 23.29 & 22.44 \\
\rowcolor{gray!20}
InternVL2.5 78B & 25.61 & 23.86 & 29.82 & 29.12 & 20.21 & 19.79 & 26.32 & 27.58 & 10.33 & 11.08 & 20.40 & 20.40 & 17.81 & 19.85 & 27.74 & 27.99 & 19.02 & 17.58 & 24.50 & 23.63 & 13.95 & 15.13 & 20.80 & 21.51 & 16.75 & 16.97 & 24.45 & 24.72 \\
Qwen2 VL 72B & 22.46 & 22.81 & 29.82 & 29.12 & 17.47 & 19.16 & 21.47 & 23.37 & 8.31 & 8.56 & 12.85 & 13.10 & 13.99 & 16.28 & 20.10 & 19.85 & 21.04 & 20.46 & 28.53 & 29.39 & 13.00 & 14.66 & 19.86 & 19.62 & 15.32 & 16.26 & 21.45 & 21.59 \\
\rowcolor{gray!20}
InternVL2.5 38B & 23.86 & 23.16 & 28.77 & 29.82 & 17.26 & 17.89 & 22.32 & 23.16 & 9.07 & 8.82 & 17.88 & 16.62 & 14.25 & 17.30 & 23.16 & 22.65 & 16.14 & 17.29 & 24.78 & 23.92 & 11.82 & 12.29 & 17.97 & 17.49 & 14.55 & 15.41 & 21.99 & 21.63 \\
Claude 3.5 Sonnet & 19.65 & 17.19 & 22.11 & 24.21 & 16.42 & 12.84 & 18.11 & 22.95 & 6.30 & 4.53 & 10.58 & 11.59 & 13.99 & 11.20 & 17.81 & 20.61 & 16.71 & 14.12 & 21.90 & 21.61 & 13.48 & 13.00 & 17.97 & 22.93 & 14.02 & 11.64 & 17.60 & 20.24 \\
\rowcolor{gray!20}
InternVL2.5 26B & 20.00 & 19.65 & 25.61 & 25.96 & 13.26 & 14.95 & 18.95 & 18.74 & 6.30 & 6.80 & 11.59 & 12.34 & 12.98 & 14.76 & 20.61 & 21.12 & 15.56 & 14.41 & 21.04 & 21.04 & 13.00 & 14.89 & 19.62 & 19.39 & 13.03 & 14.15 & 19.44 & 19.61 \\
Llama 3.2 11B Vision & 16.49 & 18.95 & 20.70 & 20.35 & 13.26 & 12.84 & 15.79 & 16.84 & 5.29 & 5.54 & 9.07 & 8.31 & 7.89 & 7.89 & 10.18 & 10.18 & 12.68 & 13.54 & 17.29 & 19.02 & 11.82 & 11.82 & 13.95 & 14.66 & 10.61 & 11.06 & 13.97 & 14.20 \\
\rowcolor{gray!20}
InternVL2.5 8B & 19.30 & 17.89 & 23.16 & 23.51 & 11.79 & 12.00 & 16.42 & 16.84 & 5.04 & 6.30 & 10.58 & 9.57 & 9.41 & 9.67 & 14.50 & 14.25 & 9.80 & 9.80 & 15.27 & 15.56 & 9.46 & 9.69 & 13.71 & 14.89 & 10.34 & 10.39 & 15.41 & 15.41 \\
Qwen2 VL 7B & 17.19 & 17.19 & 20.35 & 18.95 & 9.47 & 9.47 & 12.00 & 11.37 & 5.79 & 6.30 & 8.56 & 8.31 & 8.91 & 9.92 & 11.45 & 11.45 & 10.95 & 12.10 & 15.56 & 14.41 & 9.69 & 11.11 & 13.00 & 13.24 & 9.63 & 10.26 & 12.76 & 12.36 \\
\rowcolor{gray!20}
Phi 3.5 Vision & 14.39 & 12.63 & 20.00 & 18.95 & 8.84 & 10.74 & 13.89 & 13.47 & 6.05 & 6.05 & 8.31 & 8.82 & 6.62 & 8.14 & 9.41 & 9.92 & 8.93 & 8.65 & 14.70 & 14.70 & 8.27 & 9.93 & 13.71 & 12.77 & 8.55 & 9.18 & 12.99 & 12.85 \\
MiniCPM V 2.6 & 12.98 & 14.39 & 14.39 & 17.19 & 10.74 & 10.32 & 13.68 & 14.74 & 2.52 & 3.27 & 6.55 & 6.05 & 6.36 & 6.36 & 9.67 & 9.67 & 10.09 & 9.80 & 13.26 & 14.70 & 9.46 & 9.22 & 12.77 & 13.24 & 8.11 & 8.15 & 11.60 & 11.96 \\
\rowcolor{gray!20}
InternVL2.5 4B & 14.04 & 16.49 & 16.84 & 14.39 & 9.47 & 14.53 & 13.47 & 9.05 & 3.53 & 7.05 & 7.56 & 4.03 & 7.89 & 9.16 & 9.16 & 6.87 & 8.07 & 11.53 & 10.66 & 8.07 & 8.04 & 11.58 & 11.82 & 7.33 & 7.97 & 11.42 & 11.29 & 7.79 \\
Qwen2 VL 2B & 13.33 & 12.28 & 13.68 & 14.39 & 9.68 & 9.47 & 11.79 & 10.95 & 4.03 & 3.78 & 5.54 & 4.28 & 6.11 & 5.09 & 6.11 & 6.11 & 8.36 & 8.93 & 12.97 & 12.10 & 7.33 & 8.27 & 10.40 & 9.69 & 7.97 & 7.88 & 9.94 & 9.49 \\
\rowcolor{gray!20}
Centurio Qwen & 11.23 & 9.12 & 14.39 & 14.39 & 9.05 & 8.42 & 10.32 & 9.68 & 3.02 & 1.76 & 6.05 & 6.05 & 6.87 & 5.34 & 9.92 & 8.91 & 6.34 & 5.48 & 11.24 & 11.24 & 6.62 & 5.67 & 9.22 & 9.46 & 6.81 & 5.69 & 9.85 & 9.76 \\
InternVL2.5 2B & 6.67 & 7.37 & 10.18 & 9.47 & 4.21 & 4.63 & 6.95 & 5.89 & 2.27 & 2.02 & 3.53 & 5.29 & 2.80 & 3.56 & 5.34 & 5.60 & 3.17 & 3.75 & 7.49 & 6.92 & 5.44 & 5.44 & 8.04 & 6.15 & 4.03 & 4.39 & 6.85 & 6.45 \\
\rowcolor{gray!20}
InternVL2.5 1B & 7.02 & 7.37 & 10.53 & 11.58 & 4.21 & 3.58 & 4.84 & 4.63 & 2.52 & 0.76 & 2.77 & 2.77 & 3.56 & 3.82 & 5.09 & 4.07 & 4.61 & 3.46 & 6.63 & 7.49 & 4.02 & 5.67 & 6.86 & 6.15 & 4.03 & 4.03 & 5.96 & 5.87 \\
Centurio Aya & 3.16 & 7.37 & 8.77 & 8.77 & 2.95 & 5.68 & 9.05 & 9.68 & 1.76 & 1.51 & 4.79 & 3.53 & 1.27 & 3.56 & 5.60 & 6.11 & 2.02 & 3.46 & 7.20 & 7.20 & 2.84 & 5.44 & 6.38 & 7.09 & 2.24 & 4.39 & 6.99 & 7.17 \\
\midrule
Average X-Large & 24.04 & 23.33 & 29.82 & 29.12 & 18.84 & 19.47 & 23.89 & 25.47 & 9.32 & 9.82 & 16.62 & 16.75 & 15.90 & 18.07 & 23.92 & 23.92 & 20.03 & 19.02 & 26.51 & 26.51 & 13.48 & 14.89 & 20.33 & 20.57 & 16.03 & 16.61 & 22.95 & 23.15 \\
\rowcolor{gray!20}
Average Large & 21.93 & 21.40 & 27.19 & 27.89 & 15.26 & 16.42 & 20.63 & 20.95 & 7.68 & 7.81 & 14.74 & 14.48 & 13.61 & 16.03 & 21.88 & 21.88 & 15.85 & 15.85 & 22.91 & 22.48 & 12.41 & 13.59 & 18.79 & 18.44 & 13.79 & 14.78 & 20.71 & 20.62 \\
Average Medium & 13.39 & 14.15 & 16.96 & 17.19 & 9.54 & 9.79 & 12.88 & 13.19 & 3.90 & 4.11 & 7.60 & 6.97 & 6.79 & 7.12 & 10.22 & 10.09 & 8.65 & 9.03 & 13.30 & 13.69 & 8.31 & 8.83 & 11.51 & 12.10 & 7.96 & 8.32 & 11.76 & 11.81 \\
\rowcolor{gray!20}
Average Small & 11.09 & 11.23 & 14.25 & 13.75 & 7.28 & 8.59 & 10.19 & 8.80 & 3.68 & 3.93 & 5.54 & 5.04 & 5.39 & 5.95 & 7.02 & 6.51 & 6.63 & 7.26 & 10.49 & 9.86 & 6.62 & 8.18 & 10.17 & 8.42 & 6.51 & 7.38 & 9.40 & 8.49 \\
Average Open & 15.18 & 15.37 & 19.13 & 19.06 & 10.79 & 11.56 & 14.48 & 14.40 & 5.05 & 5.31 & 9.07 & 8.63 & 8.45 & 9.38 & 12.54 & 12.32 & 10.45 & 10.68 & 15.41 & 15.29 & 8.98 & 10.06 & 13.21 & 12.84 & 9.33 & 9.97 & 13.66 & 13.39 \\
\rowcolor{gray!20}
Average Proprietary & 24.98 & 26.67 & 30.32 & 30.39 & 21.77 & 22.48 & 27.75 & 28.55 & 12.55 & 11.64 & 21.16 & 20.35 & 18.42 & 20.31 & 26.26 & 27.12 & 21.56 & 22.19 & 29.86 & 29.74 & 18.01 & 18.58 & 23.69 & 25.20 & 19.04 & 19.84 & 26.12 & 26.53 \\
Average & 17.63 & 18.19 & 21.93 & 21.89 & 13.54 & 14.29 & 17.80 & 17.94 & 6.93 & 6.89 & 12.09 & 11.56 & 10.94 & 12.11 & 15.97 & 16.02 & 13.23 & 13.56 & 19.02 & 18.90 & 11.24 & 12.19 & 15.83 & 15.93 & 11.76 & 12.44 & 16.78 & 16.67 \\
\bottomrule
\end{tabular}

==> tables/sivqa_judge_scores.tex <==
\begin{tabular}{lrrrrrrrrrrrrrrrrrrrrrrrrrrrr}
\toprule
region & \multicolumn{4}{r}{West EU \& North America} & \multicolumn{4}{r}{Asia \& Pacific} & \multicolumn{4}{r}{Subsaharian Africa} & \multicolumn{4}{r}{Arab} & \multicolumn{4}{r}{East EU} & \multicolumn{4}{r}{Latin-America \& Caribbean} & \multicolumn{4}{r}{Average} \\
hint & N & R & C & B & N & R & C & B & N & R & C & B & N & R & C & B & N & R & C & B & N & R & C & B & N & R & C & B \\
model &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
\midrule
\rowcolor{gray!20}
GPT-4o & 55.86 & 55.46 & 64.33 & 64.49 & 56.91 & 56.42 & 63.09 & 63.20 & 39.13 & 35.97 & 48.90 & 47.93 & 51.89 & 56.53 & 65.71 & 67.59 & 54.26 & 55.62 & 67.56 & 67.33 & 48.32 & 46.69 & 53.05 & 54.09 & 51.06 & 51.12 & 60.44 & 60.77 \\
Gemini Pro & 55.44 & 56.30 & 63.15 & 62.06 & 54.23 & 54.15 & 59.84 & 59.14 & 38.74 & 39.51 & 47.63 & 46.74 & 49.83 & 52.96 & 58.10 & 57.65 & 51.67 & 52.23 & 62.48 & 63.77 & 46.54 & 45.32 & 51.95 & 52.03 & 49.41 & 50.08 & 57.19 & 56.90 \\
\rowcolor{gray!20}
Claude 3.5 Sonnet & 50.65 & 51.35 & 65.33 & 64.14 & 50.11 & 51.07 & 63.70 & 63.59 & 35.06 & 39.90 & 57.56 & 56.52 & 48.99 & 55.34 & 67.49 & 67.86 & 50.42 & 51.80 & 70.12 & 70.20 & 41.49 & 46.10 & 57.85 & 59.53 & 46.12 & 49.26 & 63.68 & 63.64 \\
Gemini Flash & 50.49 & 49.93 & 56.29 & 56.11 & 48.19 & 47.42 & 53.20 & 53.11 & 35.60 & 31.32 & 39.58 & 38.54 & 44.04 & 44.25 & 50.85 & 49.03 & 46.66 & 47.34 & 57.24 & 55.22 & 43.59 & 41.58 & 47.74 & 46.88 & 44.76 & 43.64 & 50.82 & 49.81 \\
\rowcolor{gray!20}
GPT-4o Mini & 48.98 & 48.47 & 53.10 & 54.28 & 44.83 & 44.24 & 49.96 & 49.05 & 32.78 & 35.06 & 35.49 & 35.98 & 42.24 & 43.83 & 47.98 & 48.58 & 46.57 & 43.40 & 55.06 & 53.76 & 40.74 & 38.24 & 44.21 & 44.19 & 42.69 & 42.21 & 47.63 & 47.64 \\
Qwen2 VL 72B & 40.28 & 40.05 & 48.04 & 46.90 & 38.65 & 39.25 & 43.02 & 44.15 & 25.79 & 26.30 & 31.52 & 30.57 & 32.77 & 35.27 & 42.89 & 41.64 & 38.95 & 39.44 & 50.55 & 49.74 & 30.64 & 33.06 & 39.66 & 40.27 & 34.51 & 35.56 & 42.61 & 42.21 \\
\rowcolor{gray!20}
InternVL2.5 78B & 39.88 & 39.52 & 46.43 & 47.01 & 39.93 & 38.01 & 47.78 & 49.26 & 22.18 & 20.79 & 30.15 & 30.42 & 33.72 & 35.80 & 46.82 & 47.86 & 34.57 & 32.63 & 41.89 & 40.73 & 31.42 & 30.40 & 39.09 & 38.84 & 33.62 & 32.86 & 42.03 & 42.35 \\
InternVL2.5 26B & 37.00 & 34.65 & 39.75 & 41.00 & 32.64 & 32.97 & 39.10 & 39.47 & 22.63 & 21.71 & 29.40 & 27.22 & 30.89 & 31.39 & 38.10 & 38.81 & 34.34 & 32.38 & 41.14 & 41.53 & 29.34 & 29.69 & 37.05 & 37.78 & 31.14 & 30.47 & 37.42 & 37.64 \\
\rowcolor{gray!20}
InternVL2.5 38B & 37.55 & 37.51 & 45.58 & 45.49 & 35.45 & 36.26 & 42.65 & 43.88 & 22.98 & 22.52 & 29.11 & 28.35 & 28.71 & 31.78 & 38.96 & 38.63 & 32.08 & 31.69 & 41.98 & 41.21 & 28.39 & 29.15 & 36.46 & 35.18 & 30.86 & 31.48 & 39.12 & 38.79 \\
Qwen2 VL 7B & 33.36 & 34.84 & 38.64 & 38.12 & 28.19 & 28.97 & 31.23 & 31.13 & 21.31 & 25.25 & 25.09 & 26.26 & 28.72 & 28.45 & 32.00 & 32.28 & 29.19 & 31.13 & 35.53 & 37.11 & 27.84 & 28.61 & 31.45 & 32.87 & 28.10 & 29.54 & 32.33 & 32.96 \\
\rowcolor{gray!20}
Llama 3.2 11B Vision & 35.16 & 36.56 & 37.22 & 37.81 & 27.06 & 27.59 & 31.14 & 33.09 & 19.24 & 17.97 & 24.38 & 26.42 & 25.09 & 26.53 & 31.43 & 30.47 & 28.34 & 27.88 & 33.96 & 36.73 & 26.89 & 28.82 & 32.14 & 32.88 & 26.96 & 27.56 & 31.71 & 32.90 \\
MiniCPM V 2.6 & 30.61 & 32.35 & 32.73 & 35.48 & 27.73 & 25.88 & 31.13 & 33.25 & 20.29 & 18.92 & 25.31 & 24.58 & 24.52 & 24.57 & 28.47 & 28.19 & 28.13 & 25.07 & 34.31 & 36.27 & 26.74 & 26.04 & 29.16 & 30.37 & 26.34 & 25.47 & 30.18 & 31.36 \\
\rowcolor{gray!20}
Qwen2 VL 2B & 28.86 & 28.30 & 28.94 & 30.85 & 25.18 & 24.06 & 26.32 & 26.31 & 21.02 & 19.32 & 23.06 & 21.94 & 20.92 & 20.32 & 22.98 & 23.30 & 25.10 & 26.01 & 32.90 & 31.34 & 23.91 & 24.07 & 26.73 & 25.85 & 24.16 & 23.68 & 26.82 & 26.60 \\
Centurio Aya & 29.84 & 30.21 & 30.67 & 32.31 & 26.64 & 25.51 & 28.70 & 28.81 & 18.81 & 17.87 & 21.23 & 20.97 & 19.75 & 20.43 & 24.02 & 24.01 & 25.42 & 24.93 & 28.79 & 30.72 & 23.58 & 24.65 & 25.66 & 26.68 & 24.01 & 23.93 & 26.51 & 27.25 \\
\rowcolor{gray!20}
InternVL2.5 8B & 30.12 & 32.19 & 35.35 & 36.47 & 23.62 & 23.93 & 29.75 & 29.92 & 16.70 & 17.20 & 20.54 & 21.81 & 23.61 & 23.46 & 30.65 & 29.92 & 24.94 & 24.67 & 32.73 & 33.66 & 22.80 & 22.13 & 26.78 & 27.99 & 23.63 & 23.93 & 29.30 & 29.96 \\
Phi 3.5 Vision & 24.84 & 26.93 & 33.43 & 33.45 & 23.46 & 25.36 & 29.18 & 29.02 & 21.28 & 21.65 & 23.63 & 25.92 & 21.06 & 23.26 & 26.18 & 26.48 & 24.70 & 24.88 & 31.32 & 31.82 & 24.47 & 25.73 & 29.67 & 30.56 & 23.30 & 24.64 & 28.90 & 29.54 \\
\rowcolor{gray!20}
Centurio Qwen & 27.32 & 26.32 & 29.21 & 30.42 & 25.84 & 26.54 & 26.88 & 28.63 & 18.12 & 17.91 & 20.14 & 22.69 & 23.46 & 22.32 & 27.19 & 27.72 & 20.84 & 20.56 & 26.53 & 28.83 & 21.21 & 21.74 & 23.19 & 23.82 & 22.80 & 22.56 & 25.52 & 27.02 \\
InternVL2.5 4B & 25.18 & 26.06 & 26.71 & 29.67 & 20.67 & 22.04 & 26.29 & 27.53 & 12.32 & 14.45 & 14.99 & 17.91 & 18.42 & 21.62 & 24.43 & 25.80 & 20.22 & 22.07 & 26.43 & 28.43 & 17.56 & 20.93 & 23.45 & 24.29 & 19.06 & 21.19 & 23.72 & 25.61 \\
\rowcolor{gray!20}
InternVL2.5 1B & 19.67 & 20.32 & 20.90 & 23.91 & 14.46 & 13.92 & 14.95 & 17.03 & 12.05 & 13.50 & 16.60 & 15.86 & 16.48 & 16.31 & 16.88 & 17.42 & 16.10 & 14.90 & 18.27 & 20.82 & 14.94 & 15.64 & 16.75 & 17.59 & 15.62 & 15.76 & 17.39 & 18.77 \\
InternVL2.5 2B & 18.19 & 19.35 & 20.25 & 21.95 & 14.75 & 15.99 & 16.42 & 18.36 & 13.14 & 10.52 & 12.88 & 14.96 & 15.55 & 14.08 & 16.69 & 18.03 & 14.77 & 13.73 & 17.43 & 18.32 & 15.57 & 15.86 & 18.04 & 18.77 & 15.33 & 14.92 & 16.95 & 18.40 \\
\midrule
Average X-Large & 40.08 & 39.79 & 47.23 & 46.95 & 39.29 & 38.63 & 45.40 & 46.71 & 23.99 & 23.55 & 30.83 & 30.49 & 33.25 & 35.54 & 44.86 & 44.75 & 36.76 & 36.03 & 46.22 & 45.24 & 31.03 & 31.73 & 39.37 & 39.56 & 34.06 & 34.21 & 42.32 & 42.28 \\
\rowcolor{gray!20}
Average Large & 37.28 & 36.08 & 42.67 & 43.25 & 34.05 & 34.61 & 40.88 & 41.68 & 22.81 & 22.12 & 29.25 & 27.79 & 29.80 & 31.58 & 38.53 & 38.72 & 33.21 & 32.04 & 41.56 & 41.37 & 28.86 & 29.42 & 36.75 & 36.48 & 31.00 & 30.98 & 38.27 & 38.22 \\
Average Medium & 31.07 & 32.08 & 33.97 & 35.10 & 26.51 & 26.40 & 29.80 & 30.80 & 19.08 & 19.19 & 22.78 & 23.79 & 24.19 & 24.29 & 28.96 & 28.77 & 26.14 & 25.71 & 31.98 & 33.89 & 24.84 & 25.33 & 28.06 & 29.10 & 25.31 & 25.50 & 29.26 & 30.24 \\
\rowcolor{gray!20}
Average Small & 23.35 & 24.19 & 26.05 & 27.96 & 19.70 & 20.27 & 22.63 & 23.65 & 15.96 & 15.89 & 18.23 & 19.32 & 18.48 & 19.12 & 21.43 & 22.21 & 20.18 & 20.32 & 25.27 & 26.15 & 19.29 & 20.45 & 22.93 & 23.41 & 19.49 & 20.04 & 22.76 & 23.78 \\
Average Open & 30.52 & 31.01 & 34.26 & 35.39 & 26.95 & 27.08 & 30.97 & 31.99 & 19.19 & 19.06 & 23.20 & 23.73 & 24.24 & 25.04 & 29.85 & 30.04 & 26.51 & 26.13 & 32.92 & 33.82 & 24.35 & 25.10 & 29.02 & 29.58 & 25.30 & 25.57 & 30.03 & 30.76 \\
\rowcolor{gray!20}
Average Proprietary & 52.28 & 52.30 & 60.44 & 60.22 & 50.85 & 50.66 & 57.96 & 57.62 & 36.26 & 36.35 & 45.83 & 45.14 & 47.40 & 50.58 & 58.03 & 58.14 & 49.92 & 50.08 & 62.49 & 62.05 & 44.14 & 43.59 & 50.96 & 51.34 & 46.81 & 47.26 & 55.95 & 55.75 \\
Average & 35.96 & 36.33 & 40.80 & 41.59 & 32.93 & 32.98 & 37.72 & 38.40 & 23.46 & 23.38 & 28.86 & 29.08 & 30.03 & 31.42 & 36.89 & 37.06 & 32.36 & 32.12 & 40.31 & 40.88 & 29.30 & 29.72 & 34.50 & 35.02 & 30.67 & 30.99 & 36.51 & 37.01 \\
\bottomrule
\end{tabular}

==> tables/vvqa_acc_scores.tex <==
\begin{tabular}{lrrrrrrrrrrrrrrrrrrrrrrrrrrrr}
\toprule
region & \multicolumn{4}{r}{West EU \& North America} & \multicolumn{4}{r}{Asia \& Pacific} & \multicolumn{4}{r}{Subsaharian Africa} & \multicolumn{4}{r}{Arab} & \multicolumn{4}{r}{East EU} & \multicolumn{4}{r}{Latin-America \& Caribbean} & \multicolumn{4}{r}{Average} \\
hint & N & R & C & B & N & R & C & B & N & R & C & B & N & R & C & B & N & R & C & B & N & R & C & B & N & R & C & B \\
model &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
\midrule
\rowcolor{gray!20}
GPT-4o & 38.97 & 39.91 & 41.31 & 44.13 & 34.56 & 36.41 & 35.71 & 39.17 & 23.67 & 26.33 & 36.67 & 36.00 & 29.18 & 32.46 & 36.72 & 36.39 & 37.59 & 40.43 & 47.16 & 45.74 & 31.98 & 32.56 & 38.95 & 39.24 & 32.67 & 34.49 & 39.19 & 39.97 \\
GPT-4o Mini & 38.06 & 31.58 & 34.01 & 38.87 & 29.45 & 25.64 & 25.64 & 29.66 & 20.32 & 13.33 & 15.56 & 20.63 & 28.61 & 24.40 & 25.60 & 29.52 & 35.37 & 29.27 & 30.18 & 38.72 & 25.13 & 21.20 & 23.04 & 25.65 & 28.69 & 23.89 & 24.84 & 29.69 \\
\rowcolor{gray!20}
Gemini Pro & 33.80 & 37.09 & 40.85 & 39.91 & 30.41 & 31.34 & 34.10 & 34.79 & 20.07 & 22.33 & 28.67 & 28.67 & 26.56 & 28.85 & 32.13 & 32.13 & 32.27 & 33.33 & 36.52 & 36.88 & 28.78 & 30.52 & 33.43 & 32.85 & 28.32 & 29.91 & 33.67 & 33.78 \\
Gemini Flash & 29.55 & 29.96 & 30.36 & 34.82 & 22.67 & 24.36 & 26.69 & 26.69 & 12.06 & 12.06 & 15.87 & 19.05 & 20.18 & 20.78 & 21.39 & 23.49 & 26.52 & 27.74 & 32.01 & 31.71 & 23.30 & 24.61 & 26.18 & 27.49 & 21.64 & 22.59 & 24.89 & 26.29 \\
\rowcolor{gray!20}
Claude 3.5 Sonnet & 21.86 & 19.84 & 25.91 & 24.29 & 22.46 & 19.92 & 25.21 & 25.85 & 9.21 & 6.03 & 12.38 & 11.11 & 16.87 & 14.16 & 16.87 & 18.37 & 23.17 & 20.12 & 26.52 & 24.70 & 19.11 & 15.45 & 21.47 & 22.25 & 18.74 & 15.89 & 21.44 & 21.24 \\
Qwen2 VL 72B & 25.35 & 27.23 & 33.33 & 34.27 & 18.43 & 19.12 & 23.73 & 23.73 & 9.00 & 10.00 & 16.33 & 17.00 & 17.05 & 18.36 & 22.62 & 21.64 & 25.53 & 25.53 & 32.27 & 31.91 & 16.57 & 20.93 & 23.55 & 24.42 & 18.13 & 19.62 & 24.27 & 24.65 \\
\rowcolor{gray!20}
InternVL2.5 78B & 23.94 & 29.11 & 31.92 & 31.46 & 19.12 & 24.19 & 28.11 & 29.49 & 7.33 & 12.33 & 18.67 & 19.67 & 13.44 & 22.30 & 25.90 & 25.90 & 19.50 & 24.82 & 30.14 & 29.43 & 15.41 & 21.22 & 24.42 & 26.45 & 15.75 & 21.56 & 25.98 & 26.70 \\
InternVL2.5 38B & 22.07 & 28.64 & 32.86 & 32.86 & 18.66 & 24.19 & 27.19 & 26.73 & 6.33 & 13.00 & 21.67 & 21.33 & 13.77 & 22.95 & 24.59 & 27.54 & 19.86 & 26.24 & 30.85 & 30.50 & 13.37 & 20.93 & 26.16 & 24.71 & 14.98 & 21.78 & 26.31 & 26.37 \\
\rowcolor{gray!20}
Qwen2 VL 2B & 19.72 & 18.78 & 21.13 & 23.00 & 13.13 & 14.75 & 16.59 & 15.67 & 6.67 & 4.67 & 7.00 & 6.67 & 13.11 & 11.15 & 13.44 & 12.46 & 16.67 & 16.67 & 17.38 & 17.38 & 15.70 & 15.12 & 16.28 & 16.28 & 13.88 & 13.27 & 15.26 & 14.98 \\
Qwen2 VL 7B & 18.78 & 18.78 & 22.07 & 21.60 & 14.06 & 14.06 & 17.05 & 16.59 & 5.00 & 6.00 & 7.67 & 7.33 & 13.11 & 15.08 & 17.05 & 17.70 & 15.25 & 17.73 & 18.79 & 19.50 & 15.70 & 18.60 & 19.48 & 20.06 & 13.54 & 14.76 & 16.86 & 16.92 \\
\rowcolor{gray!20}
InternVL2.5 26B & 20.66 & 25.35 & 28.64 & 29.11 & 16.36 & 19.35 & 23.27 & 24.88 & 3.33 & 7.33 & 9.33 & 10.33 & 11.80 & 15.41 & 19.67 & 20.00 & 17.73 & 21.63 & 24.82 & 24.11 & 13.66 & 18.31 & 21.51 & 22.97 & 13.32 & 17.30 & 20.78 & 21.61 \\
MiniCPM V 2.6 & 16.90 & 19.25 & 18.31 & 19.72 & 14.75 & 16.82 & 17.28 & 18.43 & 5.67 & 10.00 & 11.33 & 11.00 & 12.13 & 13.44 & 14.75 & 14.75 & 19.15 & 20.21 & 22.34 & 21.99 & 15.41 & 17.44 & 16.28 & 19.19 & 13.16 & 15.37 & 16.14 & 17.03 \\
\rowcolor{gray!20}
Phi 3.5 Vision & 16.43 & 14.55 & 16.90 & 16.90 & 13.82 & 14.06 & 17.51 & 17.28 & 8.67 & 8.33 & 10.67 & 10.33 & 9.84 & 10.16 & 11.15 & 10.82 & 15.60 & 15.25 & 19.15 & 19.86 & 13.95 & 15.12 & 18.60 & 18.90 & 12.82 & 12.88 & 16.09 & 15.87 \\
Centurio Qwen & 20.19 & 17.84 & 23.00 & 21.13 & 15.67 & 15.44 & 18.43 & 17.74 & 6.00 & 6.33 & 7.33 & 7.33 & 9.51 & 10.82 & 10.16 & 10.49 & 14.89 & 15.96 & 22.34 & 20.92 & 11.63 & 11.92 & 15.70 & 14.53 & 12.38 & 12.55 & 15.70 & 15.15 \\
\rowcolor{gray!20}
InternVL2.5 8B & 14.55 & 19.25 & 20.66 & 23.00 & 11.98 & 15.44 & 18.43 & 18.43 & 3.33 & 6.33 & 9.33 & 9.00 & 9.84 & 13.77 & 15.08 & 16.07 & 15.25 & 17.73 & 23.05 & 23.05 & 10.17 & 12.21 & 16.28 & 16.57 & 10.61 & 13.82 & 16.92 & 17.36 \\
InternVL2.5 4B & 14.55 & 15.96 & 18.78 & 18.31 & 12.67 & 14.29 & 17.74 & 16.59 & 5.67 & 6.33 & 9.00 & 9.00 & 8.52 & 9.84 & 13.11 & 12.46 & 11.35 & 15.25 & 19.50 & 18.09 & 11.34 & 14.24 & 15.70 & 15.12 & 10.45 & 12.38 & 15.70 & 14.70 \\
\rowcolor{gray!20}
Centurio Aya & 11.74 & 12.21 & 15.49 & 12.21 & 9.68 & 9.91 & 12.21 & 11.06 & 4.67 & 4.67 & 6.67 & 5.33 & 6.89 & 7.54 & 7.54 & 7.54 & 9.93 & 9.57 & 12.77 & 10.64 & 7.56 & 9.01 & 10.17 & 9.59 & 8.46 & 8.96 & 10.95 & 9.62 \\
InternVL2.5 1B & 8.45 & 9.86 & 11.27 & 12.21 & 5.76 & 8.29 & 9.22 & 7.60 & 1.67 & 2.33 & 4.00 & 2.67 & 5.90 & 7.87 & 8.85 & 8.85 & 6.74 & 7.45 & 10.99 & 10.64 & 7.27 & 8.72 & 9.01 & 9.01 & 5.86 & 7.46 & 8.90 & 8.35 \\
\midrule
Average X-Large & 24.65 & 28.17 & 32.63 & 32.86 & 18.78 & 21.66 & 25.92 & 26.61 & 8.17 & 11.17 & 17.50 & 18.33 & 15.25 & 20.33 & 24.26 & 23.77 & 22.52 & 25.18 & 31.21 & 30.67 & 15.99 & 21.08 & 23.98 & 25.44 & 16.94 & 20.59 & 25.12 & 25.68 \\
\rowcolor{gray!20}
Average Large & 21.36 & 27.00 & 30.75 & 30.99 & 17.51 & 21.77 & 25.23 & 25.81 & 4.83 & 10.17 & 15.50 & 15.83 & 12.79 & 19.18 & 22.13 & 23.77 & 18.79 & 23.94 & 27.84 & 27.30 & 13.52 & 19.62 & 23.84 & 23.84 & 14.15 & 19.54 & 23.55 & 23.99 \\
Average Medium & 16.43 & 17.46 & 19.91 & 19.53 & 13.23 & 14.33 & 16.68 & 16.45 & 4.93 & 6.67 & 8.47 & 8.00 & 10.30 & 12.13 & 12.92 & 13.31 & 14.89 & 16.24 & 19.86 & 19.22 & 12.09 & 13.84 & 15.58 & 15.99 & 11.63 & 13.09 & 15.31 & 15.21 \\
\rowcolor{gray!20}
Average Small & 14.79 & 14.79 & 17.02 & 17.61 & 11.35 & 12.85 & 15.26 & 14.29 & 5.67 & 5.42 & 7.67 & 7.17 & 9.34 & 9.75 & 11.64 & 11.15 & 12.59 & 13.65 & 16.76 & 16.49 & 12.06 & 13.30 & 14.90 & 14.83 & 10.75 & 11.50 & 13.99 & 13.47 \\
Average Open & 17.95 & 19.75 & 22.64 & 22.75 & 14.16 & 16.15 & 18.98 & 18.79 & 5.64 & 7.51 & 10.69 & 10.54 & 11.15 & 13.75 & 15.69 & 15.86 & 15.96 & 18.00 & 21.88 & 21.39 & 12.90 & 15.68 & 17.93 & 18.29 & 12.57 & 14.75 & 17.68 & 17.64 \\
\rowcolor{gray!20}
Average Proprietary & 32.45 & 31.67 & 34.49 & 36.40 & 27.91 & 27.53 & 29.47 & 31.23 & 17.06 & 16.02 & 21.83 & 23.09 & 24.28 & 24.13 & 26.54 & 27.98 & 30.98 & 30.18 & 34.48 & 35.55 & 25.66 & 24.87 & 28.61 & 29.50 & 26.01 & 25.35 & 28.80 & 30.19 \\
Average & 21.98 & 23.07 & 25.93 & 26.54 & 17.98 & 19.31 & 21.90 & 22.24 & 8.81 & 9.88 & 13.79 & 14.03 & 14.80 & 16.63 & 18.70 & 19.23 & 20.13 & 21.39 & 25.38 & 25.32 & 16.45 & 18.23 & 20.90 & 21.40 & 16.30 & 17.69 & 20.77 & 21.13 \\
\bottomrule
\end{tabular}
